How to Subvert Backdoored Encryption: Security Against Adversaries that Decrypt All Ciphertexts

We study secure and undetectable communication in a world where governments can read all encrypted communications of citizens. We consider a world where the only permitted communication method is via a government-mandated encryption scheme, using government-mandated keys. Citizens caught trying to communicate otherwise (e.g., by encrypting strings which do not appear to be natural language plaintexts) will be arrested. The one guarantee we suppose is that the government-mandated encryption scheme is semantically secure against outsiders: a perhaps advantageous feature to secure communication against foreign entities. But what good is semantic security against an adversary that has the power to decrypt? Even in this pessimistic scenario, we show citizens can communicate securely and undetectably. Informally, there is a protocol between Alice and Bob where they exchange ciphertexts that look innocuous even to someone who knows the secret keys and thus sees the corresponding plaintexts. And yet, in the end, Alice will have transmitted her secret message to Bob. Our security definition requires indistinguishability between unmodified use of the mandated encryption scheme, and conversations using the mandated encryption scheme in a modified way for subliminal communication. Our topics may be thought to fall broadly within the realm of steganography: the science of hiding secret communication in innocent-looking messages, or cover objects. However, we deal with the non-standard setting of adversarial cover object distributions (i.e., a stronger-than-usual adversary). We leverage that our cover objects are ciphertexts of a secure encryption scheme to bypass impossibility results which we show for broader classes of steganographic schemes. We give several constructions of subliminal communication schemes based on any key exchange protocol with random messages (e.g., Diffie-Hellman).

==> sections/construction.tex <==
\section{Constructions}
\label{sec:const}
In this section we describe our basic $\E-$protocol for overtly communicating a random string.  As mentioned already, here we make no assumptions about the distribution which extends realistic conversations.  In the next section we present improvements which assume some min-entropy.  We begin with a lemma which says that it suffices to construct $\E-$protocols for overtly communicating a random short string (\emph{e.g.} a single bit long), since many such protocols can be composed to get a secure protocol for overtly communicating a longer random string.

\begin{lemma}
\label{lem:comp}
Let $\E$ be a public key encryption scheme and let $\Sigma$ be an $\E-$protocol for transmitting $\eta-$bit messages.  Let $\Sigma'$ be the $\E-$protocol for transmitting $\kappa-$bit messages $(\kappa\gg\eta)$ which breaks the $\kappa-$bit string into $\eta-$bit blocks and repeatedly runs $\Sigma$.  If $\Sigma$ is overtly indistinguishable for random $\eta-$bit strings then $\Sigma'$ is overtly indistinguishable for random $\kappa-$bit strings.  Moreover, if $\Sigma$ is non-interactive then so is $\Sigma'$.
\end{lemma}

\begin{proof}
$\Sigma'$ is clearly non-interactive when $\Sigma$ is.  Overt indistinguishability of $\Sigma'$ follows from overt indistinguishability of $\Sigma$ via a simple hybrid argument.  Let $\nu=\kappa/\eta$.

\begin{enumerate}[align=left]
\item[${\sf H}_i${\bf :}] Outputs $\bigl(\sk_2,(\{c_{1,\alpha}\},\dots,\{c_{\nu,\alpha}\})\bigr)$ where random ${\sf msg}\in\{0,1\}^\kappa=\{0,1\}^{\eta\nu}$ and $\{m_{i,\alpha}\}\leftarrow\mathcal{M}^{t\nu}({\sf conv})$ are drawn and $\{c_{j,\alpha}\}\leftarrow\Sigma_1({\sf msg}_j;\pk_2;\{m_{j,\alpha}\}\bigr)$ for $j\leq i$, and $\{c_{j,\alpha}\}\leftarrow\E.\Enc(\pk_2,\{m_{j,\alpha}\})$ for $j>i$.
\end{enumerate}

\noindent
Note that ${\sf H}_0$ is the ${\sf Real}(\pk_2,\sk_2)$ distribution, while ${\sf H}_\nu$ is the ${\sf Overt}(\pk_2,\sk_2)$ distribution.  Finally, ${\sf H}_i\approx_{\sf c}{\sf H}_{i+1}$ follows from the overt indistinguishability for random $\eta-$bit messages of $\Sigma$.  Notice that the overt rate of $\Sigma'$ is $(\nu\eta)/(\nu t)$ where $\eta/t$ is the overt rate of $\Sigma$.
\end{proof}

\subsection{OK then}


\begin{definition}
\label{def:subliminal}
We say that a public-key encryption scheme $\E$ \emph{supports subliminal communication} if there exists a polynomial $r=r(\kappa)$ and a two-party $\E-$protocol $$\Pi=\bigl(\Pi_{1,1},\Pi_{1,2},\Pi_{2,1},\Pi_{2,2},\dots,\Pi_{r-1,1},\Pi_{r-1,2},\Pi_{r,1};\Pi_{2,{\sf out}}\bigr)$$ for $\kappa-$bit message transmission with the following syntax, correctness and security guarantees.

\begin{itemize}
\item \textbf{Syntax.} For each $i=1,\dots,r$, and ${\sf msg}\in\{0,1\}^\kappa$, $P_1$ draws $m_i\leftarrow\mathcal{M}(m_1,\dots,m_{i-1}')$ and $c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(\pk_1,\sk_1,\pk_2);(c_1,\dots,c_{i-1}')\bigr)$ and sends $c_i$.  Likewise for $i=1,\dots,r-1$, $P_2$ draws $m_i'\leftarrow\mathcal{M}(m_1,\dots,m_i)$ and $c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(\pk_2,\sk_2,\pk_1);(c_1,\dots,c_i)\bigr)$ and sends $c_i'$.  After $r$ rounds, $P_2$ computes ${\sf msg}'=\Pi_{2,{\sf out}}\bigl(\sk_2;(c_1,\dots,c_r)\bigr)$ and halts.

\item\textbf{Correctness.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, if $P_1$ and $P_2$ play $\Pi$ honestly, ${\sf msg}'={\sf msg}$ with probability $1-\negl(\kappa)$.

\item\textbf{Subliminal Indistinguishability.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, the following distributions are indistinguishable:

\begin{center}
\begin{tabular}{|p{0.4 \textwidth}|p{0.4\textwidth}|}
\hline
\underline{${\sf Real}(\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} & \underline{${\sf Subliminal}({\sf msg},\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} \\
{$(m_1,m_1',\dots,m_r)\leftarrow\mathcal{M}^r(\cdot)$ \newline
$c_i/c_i'\leftarrow\E.\Enc(\pk_2/\pk_1,m_i/m_i')$ \newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} &
{$m_i/m_i'\leftarrow\mathcal{M}(m_1,m_1',\dots,m_{i-1}'/m_i)$\newline
$c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(c_1,\dots,c_{i-1}')\bigr)$\newline
$c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(c_1,\dots,c_i)\bigr)$\newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} \\
\hline
\end{tabular}
\end{center}
\end{itemize}
\end{definition}

We call $\kappa/(2r-1)$ the \emph{subliminal rate} of the $\E-$protocol $\Pi$.  Note that $(2r-1)$ is the number of $\E-$ciphertexts which must be sent back and forth between $P_1$ and $P_2$ in order to subliminally communicate a $\kappa-$bit message.  

\subsection{Smuggling Encryption}
\begin{definition}[Smuggling Encryption]
	\label{def:smuggling}
For a distribution $\scS$ on $\{0,1\}^\ell$, we say that a \emph{smuggling scheme} $(\{\Hide_i\}_{i\in[n]}, \Seek)$ \emph{smuggles $\scS$} if it has the following syntax, and for any semantically secure secret-key encryption scheme $\E$, the correctness and smuggling requirements below are satisfied.

\begin{itemize}
\item \textbf{Syntax.}
Let $\Key_\kappa,\Msg_\kappa,\Ciph_\kappa$ be the key space, message space and ciphertext space of the encryption scheme, respectively.  %$\Hide_i$ and $\Seek$ work as follows.
\begin{itemize}
  \item $\Hide_i^\E$ takes $(k,m_i,s;\state_{i-1})$ as input where $(k,m_i,s)\in\Key_\kappa\times\Msg_\kappa\times\zo^\ell$, $\state_{i-1}\in\zo^*$, and outputs $(c_i,\state_i)\in\Ciph_\kappa\times\zo^*$.

  \item $\Seek^\E$ takes $(k,c_1,\dots,c_n)\in\Key_\kappa\times\Ciph_\kappa^n$ as input and outputs $s'\in\zo^\ell$.
\end{itemize}
We write $\{c_i\}\gets\Hide^\E(k,\{m_i\},s)$ to denote $\state_0=\emptyset$, $(c_i,
	\state_i)\gets\Hide_i^\E(k,m_i,s;\state_{i-1})$, $i\in[n]$. Both $\Hide$ and $\Seek$ have oracle access to the algorithms of $\E$.

\item\textbf{Correctness.} For all $(k,\{m_i\},s)\in\Key_\kappa\times\Msg_\kappa^n\times\zo^\ell$:
$$\Pr_{\{c_i\}\leftarrow\Hide^\E(k,\{m_i\},s)}\Bigl[\Seek^\E(k,\{c_i\})=s\Bigr]=1-\negl(\kappa).$$

\item\textbf{$\scS$-smuggling.} For all $\{m_i\}\in\Msg_k^n$,
%and with overwhelming probability over $k\leftarrow\E.\Gen(1^\kappa)$, 
${\sf Real}(\{m_i\})\approx_{\sf c}{\sf Smuggle}^\scS(\{m_i\})$, where the real and smuggling distributions are as follows.
%\begin{itemize}
  %\item ${\sf Real}(k,\{m_i\})$: draw $c_i\leftarrow\E.\Enc(k,m_i)$, $1\leq i\leq n$; output $(k,c_1,\dots,c_n)$.
  %\item ${\sf Smuggle}^\scS(k,\{m_i\})$: draw $s\leftarrow\scS$, $\{c_i\}\leftarrow\Hide(k,\{m_i\},s)$; output $(k,c_1,\dots,c_n)$.
%\end{itemize}
\begin{center}
\begin{tabular}{|p{0.4 \textwidth}|p{0.4\textwidth}|}
\hline
\underline{${\sf Real}(\{m_i\})${\bf :}} & \underline{${\sf Smuggle}^\scS(\{m_i\})${\bf :}} \\
{$k\leftarrow\E.\Gen(1^\kappa)$ \newline
for $1\leq i\leq n$: $c_i\leftarrow\E.\Enc(k,m_i)$ \newline
output $(k,c_1,\dots,c_n)$} &
{$k\leftarrow\E.\Gen(1^\kappa)$, $s\leftarrow\scS$ \newline
$\{c_i\}\leftarrow\Hide^\E(k,\{m_i\},s)$ \newline
output $(k,c_1,\dots,c_n)$} \\
\hline
\end{tabular}
\end{center}
\end{itemize}

\end{definition}

\paragraph{Remark.} Some remarks are in order.
\begin{enumerate}
\item It follows form the definition that $\ell, n\in\poly$. We say that $\E$ has smuggling rate $\rho$ if there exists $\Hide$, $\Seek$ as in Definition~\ref{def:smuggling} such that $\frac{\ell}{n}\geq\rho$.
\item The above secret key definition extends easily to the public key setting.  The public key syntax has each $\Hide_i$ taking the public key as input, while $\Seek$ takes the secret key. In the $\scS$-smuggling property, both keys are included in the real and smuggle distributions.
\item Note that the $\scS-$smuggling property ensures that the $c_i\leftarrow\Hide_i(k,m_i,c_1,\dots,c_{i-1})$ must be indistinguishable from an honest ciphertext $c_i\leftarrow\Enc(k,m_i)$, even given $k$.  In particular, we must have $\Dec(k,c_i)=m_i$.
\item Correctness implies that an encryption can only be $\scS-$smuggling if $\scS\approx_{\sf c}\Seek\bigl({\sf Real}(k,\{m_i\})\bigr)$, for all $\{m_i\}$ and almost all $k\leftarrow\Gen(1^\kappa)$.  Despite this limitation, we prove below that ${\sf Unif}\bigl(\zo^\ell\bigr)-$smuggling encryption implies subliminal encryption (....POSS W OTHER ASSUMPTIONS TOO?  KEY EXCH W PSRAND MSGS?...)
\end{enumerate}

\subsection{Embedding into one ciphertext at a time}
\textcolor{red}{{\bf SILAS:} proof that a ${\sf Unif}\bigl(\zo^\ell\bigr)-$smuggling encryption implies subliminal encryption here...}

\begin{proposition}
	\label{prop:product}
	Let $\scS$ be a distribution over $\zo^\ell$, and let
	$p\in\poly$. Denote by $\scS^{\otimes p}$ the product\footnote{Specifically,
	$\scS=\{\scS_{\kappa}\}_{\kappa\in\NN}$ is an ensemble of
	distributions such that for each $\kappa\in\NN$, $\scS_\kappa$ is
	a distribution over $\zo^{\ell(\kappa)}$. The product distribution
	$\scS^{\otimes p}$ is defined by considering for each $\kappa\in\NN$ the
	distribution over $(\zo^{\ell(\kappa)})^{p(\kappa)}$
	product of $p(\kappa)$ independent copies of $\scS_{\kappa}$.}
of $p$ independent copies of $\scS$. Assume that $\E$ is an $\scS$-smuggling
	encryption scheme, then $\E$ is $\scS^{\otimes p}$-smuggling. Furthermore,
	the $\scS^{\otimes p}$-smuggling rate is at least the $\scS$-smuggling
	rate.
\end{proposition}

\begin{pfsketch}
	Let $\Hide$ and $\Seek$ be as in Definition~\ref{def:smuggling}. We define
	$\Hide^{\otimes p}$ and $\Seek^{\otimes p}$ to be the concatenation of $p$
	copies of $\Hide$ and $\Seek$. Correctness of the new scheme follows from
	a simple union bound, the smuggling property follows from a standard hybrid
	argument.
\end{pfsketch}

The previous proposition implies that if $\scS$ has a product form, then to
show that an encryption scheme is $\scS$-smuggling, it is sufficient to show
that it is smuggling for a single multiplicand of the product. In particular,
if we can show that $\E$ is smuggling for uniform distributions of constant
length, then this implies that $\E$ is $\scU_\ell$-smuggling, where
$\ell\in\poly$ and $\scU_\ell\defeq\{U_{\ell(\kappa)}\}_{\kappa\in\NN}$.

\subsection{Smuggling via extractors}

We now give several constructions of smuggling schemes which use
a constant number of ciphertexts to smuggle uniform variables of constant or
logarithmic lengths. Using Proposition~\ref{prop:product}, this implies
smuggling of uniform variables of arbitrary polynomial length with a constant
or logarithmic rate.

\begin{definition}\label{def:2ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^c$, and let
	$\TwoExt:\zo^c\times\zo^c\to\zo^\ell$ be a two-source extractor.
	We define a smuggling scheme for strings of length $\ell$, as follows.
\begin{itemize}
  \item $\Hide_1$ takes as input $(k,m_1,s)$, samples $c_1\gets\E.\Enc(k,m)$, and outputs $(c_1,c_1)$.
  \item $\Hide_2$ takes as input $(k,m_2,s, c_1)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt2} Sample encryption $c_2\gets\E.\Enc(k,m)$.
      \item If $\Ext(c_1,c_2)=s$, then output $c_2$. Else, go back to step \ref{itm:encrypt2}.
    \end{enumerate}
  \item $\Seek$ takes as input $(k,c_1,c_2)$ and outputs $s':=\Ext(c_1,c_2)$.
\end{itemize}
\end{definition}

\begin{remark}
The scheme of Definitions \ref{def:2ext_rejsampling} is only \emph{expected}
	polynomial time.  It could straightforwardly be modified to run in
	polynomial time, by setting a polynomial upper bound on the number of
	attempted encryptions.  For an appropriate setting of this upper bound
	(e.g., $\ell^2$), the distance between the output distribution of the
	original and modified (upper-bounded) algorithms would be negligible.
\end{remark}


==> sections/extractors.tex <==
\section{Deterministic extraction of ciphertexts}

Our constructions of embedding schemes rely on the ability to extract
randomness from ciphertexts. Ideally, we would use single explicit family of
functions $\Ext$ whose output has negligible bias when computed on ciphertexts
of \emph{any} semantically secure encryption scheme. As we show in
Lemma~\ref{lemma:cond-min-ent}, ciphertexts of secure schemes have min-entropy
$\omega(\log \kappa)$, so the above requirement would be met if for any
$d\in\NN$, $\Ext$ had bias at most $\frac{1}{\kappa^d}$ for all sources of
min-entropy at least $d\log\kappa$.

However, it is well-known (see \emph{e.g.} Proposition 6.11 in \cite{vad10})
that such a family does not exist.  Specifically, for any deterministic
function $\Ext:\zo^n\to\zo$, there exists a source $X$ with $\Me(X)\geq n-1$
and such that $\Ext(X)$ is constant. In Proposition~\ref{prop:impossibility},
we show that a similar impossibility result holds even if we restrict the class
of sources to ciphertexts of secure encryption schemes.

The way we bypass this impossibility result is by:
\begin{itemize}
	\item either allowing the extractor to depend on the encryption scheme by
		using the deterministic extractor of \cite{trevad} for efficiently
		samplable distributions.
	\item or extracting from more than one source: multiple ciphertexts or
		pairs of (message, ciphertext).
\end{itemize}
Note that the usual way of bypassing the impossibility of deterministic
extraction by considering seeded extractors is not acceptable since our
constructions require the two parties to evaluate the same extractor. For
seeded extractors, this would require the seed to be either a shared secret or
a common random string.

\iffalse
\begin{definition}
	\label{def:ext}
	The family $\Ext
	= \{\Ext_{\kappa}:\zo^{n(\kappa)}\to\zo^{\ell(\kappa)}\}_{\kappa\in\NN}$ is
	a $(k,\eps)$-\emph{extractor} if for all $\kappa\in\NN$ and for all random
	variable $X$ over $\zo^{n(\kappa)}$ such that $\Me(X)\geq k(\kappa)$:
	\begin{displaymath}
		\sdist{\Ext_{\kappa}(X)-U_{\ell(\kappa)}}\leq \eps(\kappa).
	\end{displaymath}
	Furthermore, we say that $\Ext$ is \emph{explicit} if there exists
	a polynomial time (uniform) algorithm $A$ such that:
	\begin{displaymath}
		\forall \kappa\in\NN,\; \forall x\in\zo^{n(\kappa)},\;
		A(x) = \Ext_{\kappa}(x).
	\end{displaymath}
\end{definition}

\begin{remark}
	When there is no ambiguity, we will abuse notations and write statements
	such as ``$\Ext:\zo^n\to\zo^\ell$ is a $(k,\eps)$ extractor'' where the
	dependency on $\kappa$ is implicit.
\end{remark}
\fi

\iffalse
\begin{lemma}
	Let $\PKE$ be a semantically secure encryption scheme with message length
	$n$ and ciphertext length $c$. Let $\Ext:\zo^c\to\zo^\ell$ be a $(n, \eps)$
	extractor for some negligible function $\eps$, then writing $(PK,
	SK)\sim\PKE.\Gen$, $C_m\sim\PKE.\Enc(PK, m)$, we have $\Ext(C_m)\compIndist
	U_\ell$.
\end{lemma}

\begin{proof}
	Let $\sD:\zo^\ell\to\zo$ be a distinguisher, by semantic security there
	exists a negligible function $\eps'$ such that for all $(m_0,m_1)\in\Msg^2$:
	\begin{displaymath}
		\Dist_{C_{m_{0}},C_{m_{1}}}(\sD\circ\Ext)\leq\eps'.
	\end{displaymath}

	Let us define $Y\sim\PKE.\Enc(PK,U_n)$, then for any $m\in\Msg$:
	\begin{displaymath}
		\Dist_{C_m,Y}(\sD\circ\Ext)
		\leq\frac{1}{2^n}\sum_{m'\in\Msg}
		\Dist_{C_m,C_{m'}}(\sD\circ\Ext)=\eps'
		\;,
	\end{displaymath}
	where the first inequality uses the definition of $Y$ and the triangle
	inequality.

	Observe that for all $(pk, sk)\gets\PKE.\Gen(1^k)$, by correctness of
	$\PKE$, $\PKE.\Enc(pk, U_n)$ is a flat source supported on a set of size
	$2^{n(\kappa)}$, hence $\Me(Y)\geq n$. We can then write:
	\begin{displaymath}
		\big| \Pr[\sD(\Ext(C_m))=1] - \Pr[\sD(U_\ell)=1] \big|
		\leq
		\Dist_{C_m,Y}(\sD\circ\Ext) + \sdist{\Ext(Y)-U_\ell}\leq\eps'+\eps
		\;,
	\end{displaymath}
	where the first inequality follows from the triangle inequality and the
	definition of statistical distance.
\end{proof}
\fi


==> sections/genmodel.tex <==
\section{(generalized model)}\label{sec:genmodel}

We can generalize the definition from \ref{sec:model} to capture a notion of "hiding" also in the case that the messages are not arbitrary, but are drawn from some distribution(s).
This may seem like a weaker definition; however, for arbitrary distributions, it is in fact more general.

\subsection{Conversation distributions}

For simplicity, we only consider conversations involving two parties, $A$ and $B$,
but our results extend to conversations between multiple parties.
We assume a synchronous communication model in which every party may send a message in every round.
A communication \emph{transcript} consists of a list of the messages
sent by each party for a number of consecutive rounds of communication.
We assume there is a PKI that provides a unique public identifier to each party.

\begin{definition}[Next-message algorithm]
A \emph{next-message algorithm} $\Next$ for message space $\Msg$
is a PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
and outputs a ``next message'' $m\in\Msg\cup\{\bot\}$, where the $\bot$ symbol denotes that no message is to be sent in the next round.
\end{definition}

%\begin{definition}[Next-ciphertext algorithm]
%For any encryption scheme $\E$, we denote by $\Next^{\E,k}$ the PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
%samples $m\gets\Next(\tau)$, and outputs an encryption $\E.\Enc(k,m)$.
%\end{definition}

\begin{definition}[Plaintext conversation distribution]
%Let $\PKE$ be a public-key encryption scheme and
Let $(A,B)$ be a pair of parties with public keys $pk_A,pk_B$ respectively,
and with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Then there is induced a unique \emph{$N$-round conversation distribution} $\Convo_{N,\Nextvec}$
defined by the following sampling procedure:

\begin{enumerate}
\item Initialize $\btau:=()$ to be an empty list.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  %\item\label{step:msg_i} Let $\tau_i:=(m_A,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \end{enumerate}
\item Output $\btau$.
\end{enumerate}
\end{definition}

\begin{definition}[Encrypted conversation distribution]
Let $(A,B)$ be a pair of parties %with public keys $pk_A,pk_B$ respectively,
with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Let $\E$ be an encryption scheme and let $k_A,k_B$ be encryption keys thereof.
There is induced an \emph{$N$-round encrypted conversation distribution} $\Convo_{N,\Nextvec}^{\E,k_A,k_B}$
defined by the following sampling procedure:
%same message-sampling procedure as above, except with step \ref{step:msg_i} replaced by the following:
%\begin{itemize}
%\item Sample $c_A\gets\PKE.\Enc(pk_B,m_A)$ and $c_B\gets\PKE.\Enc(pk_A,m_B)$ and let $\tau_i:=(c_A,c_B)$.
%\end{itemize}

\begin{enumerate}
\item Initialize $\btau:=(),\btau':=()$.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  \item Sample $c_A\gets\SKE.\Enc(sk,m_A)$ and $c_B\gets\SKE.\Enc(sk,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \item Append $(c_A,c_B)$ to the (encrypted) transcript $\btau'$.
  \end{enumerate}
\item Output $\btau'$.
\end{enumerate}
\end{definition}

\sunoo{indistinguishability definition}



==> sections/model.tex <==

\section{Subliminal Communication}\label{sec:model}
\begin{definition}
\label{def:subliminal}
We say that a public-key encryption scheme $\E$ \emph{supports subliminal communication} if there exists a polynomial $r=r(\kappa)$ and a two-party $\E-$protocol $$\Pi=\bigl(\Pi_{1,1},\Pi_{1,2},\Pi_{2,1},\Pi_{2,2},\dots,\Pi_{r-1,1},\Pi_{r-1,2},\Pi_{r,1};\Pi_{2,{\sf out}}\bigr)$$ for $\kappa-$bit message transmission with the following syntax, correctness and security guarantees.

\begin{itemize}
\item \textbf{Syntax.} For each $i=1,\dots,r$, and ${\sf msg}\in\{0,1\}^\kappa$, $P_1$ draws $m_i\leftarrow\mathcal{M}(m_1,\dots,m_{i-1}')$ and $c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(\pk_1,\sk_1,\pk_2);(c_1,\dots,c_{i-1}')\bigr)$ and sends $c_i$.  Likewise for $i=1,\dots,r-1$, $P_2$ draws $m_i'\leftarrow\mathcal{M}(m_1,\dots,m_i)$ and $c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(\pk_2,\sk_2,\pk_1);(c_1,\dots,c_i)\bigr)$ and sends $c_i'$.  After $r$ rounds, $P_2$ computes ${\sf msg}'=\Pi_{2,{\sf out}}\bigl(\sk_2;(c_1,\dots,c_r)\bigr)$ and halts.

\item\textbf{Correctness.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, if $P_1$ and $P_2$ play $\Pi$ honestly, ${\sf msg}'={\sf msg}$ with probability $1-\negl(\kappa)$.

\item\textbf{Subliminal Indistinguishability.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, the following distributions are indistinguishable:

\begin{center}
\begin{tabular}{|p{0.4 \textwidth}|p{0.4\textwidth}|}
\hline
\underline{${\sf Real}(\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} & \underline{${\sf Subliminal}({\sf msg},\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} \\
{$(m_1,m_1',\dots,m_r)\leftarrow\mathcal{M}^r(\cdot)$ \newline
$c_i/c_i'\leftarrow\E.\Enc(\pk_2/\pk_1,m_i/m_i')$ \newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} &
{$m_i/m_i'\leftarrow\mathcal{M}(m_1,m_1',\dots,m_{i-1}'/m_i)$\newline
$c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(c_1,\dots,c_{i-1}')\bigr)$\newline
$c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(c_1,\dots,c_i)\bigr)$\newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} \\
\hline
\end{tabular}
\end{center}
\end{itemize}
\end{definition}

We call $\kappa/(2r-1)$ the \emph{subliminal rate} of the $\E-$protocol $\Pi$.  Note that $(2r-1)$ is the number of $\E-$ciphertexts which must be sent back and forth between $P_1$ and $P_2$ in order to subliminally communicate a $\kappa-$bit message.  

\subsection{Smuggling Encryption}
\begin{definition}[Smuggling Encryption]
	\label{def:smuggling}
For a distribution $\scS$ on $\{0,1\}^\ell$, we say that a \emph{smuggling scheme} $(\{\Hide_i\}_{i\in[n]}, \Seek)$ \emph{smuggles $\scS$} if it has the following syntax, and for any semantically secure secret-key encryption scheme $\E$, the correctness and smuggling requirements below are satisfied.

\begin{itemize}
\item \textbf{Syntax.}
Let $\Key_\kappa,\Msg_\kappa,\Ciph_\kappa$ be the key space, message space and ciphertext space of the encryption scheme, respectively.  %$\Hide_i$ and $\Seek$ work as follows.
\begin{itemize}
  \item $\Hide_i^\E$ takes $(k,m_i,s;\state_{i-1})$ as input where $(k,m_i,s)\in\Key_\kappa\times\Msg_\kappa\times\zo^\ell$, $\state_{i-1}\in\zo^*$, and outputs $(c_i,\state_i)\in\Ciph_\kappa\times\zo^*$.

  \item $\Seek^\E$ takes $(k,c_1,\dots,c_n)\in\Key_\kappa\times\Ciph_\kappa^n$ as input and outputs $s'\in\zo^\ell$.
\end{itemize}
We write $\{c_i\}\gets\Hide^\E(k,\{m_i\},s)$ to denote $\state_0=\emptyset$, $(c_i,
	\state_i)\gets\Hide_i^\E(k,m_i,s;\state_{i-1})$, $i\in[n]$. Both $\Hide$ and $\Seek$ have oracle access to the algorithms of $\E$.

\item\textbf{Correctness.} For all $(k,\{m_i\},s)\in\Key_\kappa\times\Msg_\kappa^n\times\zo^\ell$:
$$\Pr_{\{c_i\}\leftarrow\Hide^\E(k,\{m_i\},s)}\Bigl[\Seek^\E(k,\{c_i\})=s\Bigr]=1-\negl(\kappa).$$

\item\textbf{$\scS$-smuggling.} For all $\{m_i\}\in\Msg_k^n$,
%and with overwhelming probability over $k\leftarrow\E.\Gen(1^\kappa)$, 
${\sf Real}(\{m_i\})\approx_{\sf c}{\sf Smuggle}^\scS(\{m_i\})$, where the real and smuggling distributions are as follows.
%\begin{itemize}
  %\item ${\sf Real}(k,\{m_i\})$: draw $c_i\leftarrow\E.\Enc(k,m_i)$, $1\leq i\leq n$; output $(k,c_1,\dots,c_n)$.
  %\item ${\sf Smuggle}^\scS(k,\{m_i\})$: draw $s\leftarrow\scS$, $\{c_i\}\leftarrow\Hide(k,\{m_i\},s)$; output $(k,c_1,\dots,c_n)$.
%\end{itemize}
\begin{center}
\begin{tabular}{|p{0.4 \textwidth}|p{0.4\textwidth}|}
\hline
\underline{${\sf Real}(\{m_i\})${\bf :}} & \underline{${\sf Smuggle}^\scS(\{m_i\})${\bf :}} \\
{$k\leftarrow\E.\Gen(1^\kappa)$ \newline
	for $1\in[n]$: $c_i\leftarrow\E.\Enc(k,m_i)$ \newline
output $(k,c_1,\dots,c_n)$} &
{$k\leftarrow\E.\Gen(1^\kappa)$, $s\leftarrow\scS$ \newline
$\{c_i\}\leftarrow\Hide^\E(k,\{m_i\},s)$ \newline
output $(k,c_1,\dots,c_n)$} \\
\hline
\end{tabular}
\end{center}
\end{itemize}

\end{definition}

\paragraph{Remark.} Some remarks are in order.
\begin{enumerate}
\item It follows form the definition that $\ell, n\in\poly$. The rate of
	a smuggling scheme is defined by $\rho\defeq\frac{\ell}{n}$.
\item The above secret key definition extends easily to the public key setting.  The public key syntax has each $\Hide_i$ taking the public key as input, while $\Seek$ takes the secret key. In the $\scS$-smuggling property, both keys are included in the real and smuggle distributions.
\item Note that the $\scS$-smuggling property ensures that the $c_i\leftarrow\Hide_i(k,m_i,c_1,\dots,c_{i-1})$ must be indistinguishable from an honest ciphertext $c_i\leftarrow\Enc(k,m_i)$, even given $k$.  In particular, we must have $\Dec(k,c_i)=m_i$.
\item Correctness implies that an encryption can only be $\scS$-smuggling if $\scS\approx_{\sf c}\Seek\bigl({\sf Real}(k,\{m_i\})\bigr)$, for all $\{m_i\}$ and almost all $k\leftarrow\Gen(1^\kappa)$.  Despite this limitation, we prove below that ${\sf Unif}\bigl(\zo^\ell\bigr)-$smuggling encryption implies subliminal encryption (....POSS W OTHER ASSUMPTIONS TOO?  KEY EXCH W PSRAND MSGS?...)
\end{enumerate}

\begin{proposition}
	\label{prop:product}
	Let $\scS$ be a distribution over $\zo^\ell$, and let $p\in\poly$. Denote
	by $\scS^{\otimes p}$ the product\footnote{Specifically,
	$\scS=\{\scS_{\kappa}\}_{\kappa\in\NN}$ is an ensemble of distributions
	such that for each $\kappa\in\NN$, $\scS_\kappa$ is a distribution over
	$\zo^{\ell(\kappa)}$. The product distribution $\scS^{\otimes p}$ is
	defined by considering for each $\kappa\in\NN$ the distribution over
	$(\zo^{\ell(\kappa)})^{p(\kappa)}$ product of $p(\kappa)$ independent
	copies of $\scS_{\kappa}$.} of $p$ independent copies of $\scS$. If there
	exsists an $\scS$-smuggling scheme, then there exists an $\scS^{\otimes
	p}$-smuggling scheme. Furthermore, the rates of both schemes are equal.
\end{proposition}

\tbo{In cases where the first Hide function does nothing, we can have
a slightly more efficient "product theorem" by replacing it with the output of
the last hide of the previous multiplicand of the product, effectively
overlapping the repetitions of the smuggling scheme. To be written if we have
enough time.}

\begin{pfsketch}
	Let $\Hide$ and $\Seek$ be as in Definition~\ref{def:smuggling}. We define
	$\Hide^{\otimes p}$ and $\Seek^{\otimes p}$ to be the concatenation of $p$
	copies of $\Hide$ and $\Seek$. Correctness of the new scheme follows from
	a simple union bound, the smuggling property follows from a standard hybrid
	argument.
\end{pfsketch}

The previous proposition implies that if $\scS$ has a product form, then to
construct an $\scS$-smuggling scheme, then it is sufficient to construct
a smuggling scheme for a single multiplicand of the product. In particular, if
there exists a smuggling scheme for a constant number of uniformly random bits,
then there exists a $\scU_\ell$-smuggling scheme for $\ell\in\poly$ where
$\scU_\ell\defeq\{U_{\ell(\kappa)}\}_{\kappa\in\NN}$.

\subsection{Smuggling via extractors}\label{sec:construction}

We now give a construction of a smuggling scheme which uses pairs of ciphertexts to smuggle uniform variables of constant or
logarithmic lengths. Using Proposition~\ref{prop:product}, this implies
smuggling of uniform variables of arbitrary polynomial length with a constant
or logarithmic rate.

\begin{definition}\label{def:2ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^n$, and let
	$\TwoExt:\zo^n\times\zo^n\to\zo^\ell$ be a two-source extractor.
	We define a smuggling scheme for strings of length $\ell$, as follows.
\begin{itemize}
  \item $\Hide_1$ takes as input $(pk,m_1,s; \emptyset)$, samples
	  $c_1\gets\E.\Enc(pk,m_1)$, and outputs $(c_1,c_1)$.
  \item $\Hide_2$ takes as input $(pk,m_2,s; c_1)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt2} Sample encryption $c_2\gets\E.\Enc(pk,m)$.
	  \item If $\TwoExt(c_1,c_2)=s$, then output $(c_2, \emptyset)$. Else, go
		  back to step \ref{itm:encrypt2}.
    \end{enumerate}
  \item $\Seek$ takes as input $(pk,c_1,c_2)$ and outputs
	  $s':=\TwoExt(c_1,c_2)$.
\end{itemize}
\end{definition}

\begin{remark}
The scheme of Definitions \ref{def:2ext_rejsampling} is only \emph{expected}
	polynomial time.  It could straightforwardly be modified to run in
	polynomial time, by setting a polynomial upper bound on the number of
	attempted encryptions.  For an appropriate setting of this upper bound
	(e.g., $\ell^2$), the distance between the output distribution of the
	original and modified (upper-bounded) algorithms would be negligible.
\end{remark}

\begin{proposition}
	Assume that $\ell(\kappa)=O(\log\kappa)$ and that
	$\TwoExt:\zo^n\times\zo^n\to\zo^\ell$ is a same-source extractor for
	super-logarithmic min-entropy, then the construction of
	Definition~\ref{def:2ext_rejsampling} is a $\scU_\ell$-smuggling scheme.
\end{proposition}

\begin{proof}
	Let $m_1$, $m_2$ be two messages. Let us define the following random
	variables:
	\begin{gather*}
		(PK, SK)=\Gen(1^\kappa)\;,\\
		C_1 = \Enc(PK, m_1)\quad (C_1',C_1')=\Hide_1(PK, m_1, U_{\ell(\kappa)};\emptyset)\;,\\
		C_2,D_2\stackrel{i.i.d.}{\sim} \Enc(PK, m_2)
		\quad (C_2',\emptyset)=\Hide_2(PK, m_2, U_{\ell(\kappa)};C_1')
	\end{gather*}
	Note that by definition of $\Hide_1$, $C_1'\sim C_1$ and that by
	definition of $\Hide_2$:
	\begin{displaymath}
		(C_2,\emptyset) \sim \Hide_2\big(PK, m_2, \TwoExt(C_1, D_2); C_1\big)
	\end{displaymath}
	But by Lemma~\ref{lemma:2ext-comp}, we have:
	\begin{displaymath}
		\sdist{\big(PK, SK, C_1, \TwoExt(C_1, D_2)\big)
		-(PK, SK, C_1', U_{\ell(\kappa)})}
		\leq \eps(\kappa)\;.
	\end{displaymath}
	The statistical distance can only decrease by applying $\Hide_2$, hence:
	\begin{displaymath}
		\sdist{(PK, SK, C_1, C_2)
		-(PK, SK, C_1', C_2')}
		\leq \eps(\kappa)\;.\qedhere
	\end{displaymath}
\end{proof}

\begin{definition}\label{def:ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^n$, and let
	$\Ext:\zo^n\to\zo^\ell$ be a deterministic extractor.
We define a smuggling scheme for strings of length $\ell$, as follows.

\begin{itemize}
  \item $\Hide$ takes as input $(k,m,s;\emptyset)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt1} Sample encryption $c\gets\E.\Enc(k,m)$.
	  \item If $\Ext(c)=s$, then output $c$. Else, go back to step
		  \ref{itm:encrypt1}.
    \end{enumerate}
  \item $\Seek$ takes as input $(k,c)$ and outputs $s':=\Ext(c)$.
\end{itemize}
\end{definition}

\sunoo{possible remark 1: can use multi-source extractor. with current constructions, there is no point (assuming that we "overlap pairs")}

\sunoo{possible remark 2: XOR trick (but maybe it can just stay in the intro)}

\subsection{Leveraging succinct encryption for better smuggling rate}

\tbo{include HILL entropy argument with 2-source extractor (note: can exploit entropy from both sources). 
BUT omit the Luca-Salil version for now (maybe add after submission?)}

==> sections/oldmodel.tex <==
For simplicity, we only consider conversations involving two parties, $A$ and $B$,
but our results extend to conversations between multiple parties.
We assume a synchronous communication model in which every party may send a message in every round.
A communication \emph{transcript} consists of a list of the messages
sent by each party for a number of consecutive rounds of communication.
We assume there is a PKI that provides a unique public identifier to each party.

\begin{definition}[Next-message algorithm]
A \emph{next-message algorithm} $\Next$ for message space $\Msg$
is a PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
and outputs a ``next message'' $m\in\Msg\cup\{\bot\}$, where the $\bot$ symbol denotes that no message is to be sent in the next round.
\end{definition}

%\begin{definition}[Next-ciphertext algorithm]
%For any encryption scheme $\E$, we denote by $\Next^{\E,k}$ the PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
%samples $m\gets\Next(\tau)$, and outputs an encryption $\E.\Enc(k,m)$.
%\end{definition}

\begin{definition}[Plaintext conversation distribution]
%Let $\PKE$ be a public-key encryption scheme and
Let $(A,B)$ be a pair of parties with public keys $pk_A,pk_B$ respectively,
and with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Then there is induced a unique \emph{$N$-round conversation distribution} $\Convo_{N,\Nextvec}$
defined by the following sampling procedure:

\begin{enumerate}
\item Initialize $\btau:=()$ to be an empty list.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  %\item\label{step:msg_i} Let $\tau_i:=(m_A,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \end{enumerate}
\item Output $\btau$.
\end{enumerate}
\end{definition}

\begin{definition}[Encrypted conversation distribution]
Let $(A,B)$ be a pair of parties %with public keys $pk_A,pk_B$ respectively,
with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Let $\E$ be an encryption scheme and let $k_A,k_B$ be encryption keys thereof.
There is induced an \emph{$N$-round encrypted conversation distribution} $\Convo_{N,\Nextvec}^{\E,k_A,k_B}$
defined by the following sampling procedure:
%same message-sampling procedure as above, except with step \ref{step:msg_i} replaced by the following:
%\begin{itemize}
%\item Sample $c_A\gets\PKE.\Enc(pk_B,m_A)$ and $c_B\gets\PKE.\Enc(pk_A,m_B)$ and let $\tau_i:=(c_A,c_B)$.
%\end{itemize}

\begin{enumerate}
\item Initialize $\btau:=(),\btau':=()$.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  \item Sample $c_A\gets\SKE.\Enc(sk,m_A)$ and $c_B\gets\SKE.\Enc(sk,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \item Append $(c_A,c_B)$ to the (encrypted) transcript $\btau'$.
  \end{enumerate}
\item Output $\btau'$.
\end{enumerate}
\end{definition}

\subsection{Embedding into one ciphertext at a time}

\begin{definition}[Simple embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$.
A \emph{simple embedding scheme for strings of length $\ell$} is a pair of algorithms $\Sigma=(\Sigma.\Hide,\Sigma.\Seek)$ as follows.
\begin{itemize}
  \item $\Sigma.\Hide$ takes as input a key $k$, message $m\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs a ciphertext $c\in\Ciph_\kappa$.
  \item $\Sigma.\Seek$ takes as input a key $k'$ and a ciphertext $c\in\Ciph_\kappa$, and outputs a string $s'\in\zo^{\ell(\kappa)}$.
\end{itemize}
%We say that $\Sigma$ is \emph{secure w.r.t. $\SKE$ (respectively, $\PKE$)}
%if it is \emph{correct} and \emph{hiding} w.r.t. $\SKE$ (respectively, $\PKE$) as defined below.
\end{definition}

\begin{definition}[Correctness of simple embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$,
and let $\Sigma$ be a simple embedding scheme for strings of length $\ell=\ell(\kappa)$.
\begin{itemize}
  \item $\Sigma$ is \emph{correct w.r.t. $\SKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell,m\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    sk\gets\SKE.\Gen(1^\kappa) \\
    c\gets\Sigma.\Hide(sk,m,s) \\
    s'\gets\Sigma.\Seek(sk,c)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
  \item $\Sigma$ is \emph{correct w.r.t. $\PKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell,m\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    (pk,sk)\gets\PKE.\Gen(1^\kappa) \\
    c\gets\Sigma.\Hide(pk,m,s) \\
    s'\gets\Sigma.\Seek(sk,c)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
\end{itemize}
\end{definition}

\begin{definition}[Hiding of simple embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
A simple embedding scheme $\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\SKE.\Enc(sk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(sk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\PKE.\Enc(pk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(pk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}

\subsection{Adaptive embedding into pairs of ciphertexts}

\begin{definition}[Two-part embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$.
A \emph{two-part embedding scheme for strings of length $\ell$} is a triple of algorithms $\Sigma=(\Sigma.\Hide_1,\Sigma.\Hide_2,\Sigma.\Seek)$ as follows.
\begin{itemize}
  \item $\Sigma.\Hide_1$ takes as input a key $k$, message $m_1\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs $(c_1,\state)$ where $c_1\in\Ciph_\kappa$ is a ciphertext and $\state\in\zo^*$ is a \emph{state}.
  \item $\Sigma.\Hide_2$ takes as input a state $\state$, a key $k$, message $m_2\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs a ciphertext $c_2\in\Ciph_\kappa$.
  \item $\Sigma.\Seek$ takes as input a key $k$ and ciphertexts $c_1,c_2\in\Ciph_\kappa)$, and outputs a string $s'\in\zo^{\ell(\kappa)}$.
\end{itemize}
\end{definition}

\begin{definition}[Correctness of two-part embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$,
and let $\Sigma$ be a two-part embedding scheme for strings of length $\ell=\ell(\kappa)$.
\begin{itemize}
  \item $\Sigma$ is \emph{correct w.r.t. $\SKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell$ and $m_1,m_2\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    sk\gets\SKE.\Gen(1^\kappa) \\
    (c_1,\state)\gets\Sigma.\Hide_1(sk,m_1,s) \\
    c_2\gets\Sigma.\Hide_2(\state,sk,m_2,s) \\
    s'\gets\Sigma.\Seek(sk,c_1,c_2)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
  \item $\Sigma$ is \emph{correct w.r.t. $\PKE$} if there is a negligible function $\eps$ such that for all $s\in\zo^\ell$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    (pk,sk)\gets\PKE.\Gen(1^\kappa) \\
    (c_1,\state)\gets\Sigma.\Hide_1(pk,m_1,s) \\
    c_2\gets\Sigma.\Hide_2(\state,pk,m_2,s) \\
    s'\gets\Sigma.\Seek(sk,c_1,c_2)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
\end{itemize}
\end{definition}

\begin{definition}[Hiding of two-part embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
A two-part embedding scheme $\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $((m_{1,1},m_{1,2}),\dots,(m_{N,1},m_{N,2}))\in((\Msg_\kappa)^2)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_{0,1}\gets\SKE.\Enc(sk,m_{i,1}) \\
\forall i\in[N], ~ c^{(i)}_{0,2}\gets\SKE.\Enc(sk,m_{i,2}) \\
\forall i\in[N], ~ (c^{(i)}_{1,1},\state_i)\gets\Sigma.\Hide_1(sk,m_{i,1},s_i) \\
\forall i\in[N], ~ c^{(i)}_{1,2}\gets\Sigma.\Hide_2(\state_i,sk,m_{i,2},s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $((m_{1,1},m_{1,2}),\dots,(m_{N,1},m_{N,2}))\in((\Msg_\kappa)^2)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_{0,1}\gets\PKE.\Enc(pk,m_{i,1}) \\
\forall i\in[N], ~ c^{(i)}_{0,2}\gets\PKE.\Enc(pk,m_{i,2}) \\
\forall i\in[N], ~ (c^{(i)}_{1,1},\state_i)\gets\Sigma.\Hide_1(pk,m_{i,1},s_i) \\
\forall i\in[N], ~ c^{(i)}_{1,2}\gets\Sigma.\Hide_2(\state_i,pk,m_{i,2},s_i) \\
b'\gets\sD(sk,(c^{(1)}_{b,1},c^{(1)}_{b,2}),\dots,(c^{(N)}_{b,1},c^{(N)}_{b,2})) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}

\begin{remark}
One could consider extending this definition to embed in more than polynomially many (rather than just two) ciphertexts at a time.
\sunoo{mention why adaptivity is important}
\end{remark}

\iffalse
\begin{definition}[Hiding of string-embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
$\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\SKE.\Enc(sk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(sk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\PKE.\Enc(pk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(pk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}
\fi

\subsection{Embedding schemes based on extractors}

\begin{definition}\label{def:ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^c$, and let
	$\Ext:\zo^c\to\zo^\ell$ be a deterministic extractor.
We define a simple embedding scheme $\Sigma^{\E,\Ext}$ for strings of length $\ell$, as follows.
\begin{itemize}
  \item $\Sigma^{\E,\Ext}.\Hide$ takes as input $(k,m,s)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt1} Sample encryption $c\gets\E.\Enc(k,m)$.
      \item If $\Ext(c)=s$, then output $c$. Else, go back to step \ref{itm:encrypt1}.
    \end{enumerate}
  \item $\Sigma^{\E,\Ext}.\Seek$ takes as input $(k',c)$ and outputs $s':=\Ext(c)$.
\end{itemize}
\end{definition}

\begin{definition}\label{def:2ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^c$, and let
	$\TwoExt:\zo^c\times\zo^c\to\zo^\ell$ be a two-source extractor.
	We define
	a string-embedding scheme $\Sigma^{\E,\TwoExt}$ for strings of length
	$\ell$, as follows.
\begin{itemize}
  \item $\Sigma^{\E,\TwoExt}.\Hide_1$ takes as input $(k,m_1,s)$, samples $c_1\gets\E.\Enc(k,m)$, and outputs $(c_1,c_1)$.
  \item $\Sigma^{\E,\TwoExt}.\Hide_2$ takes as input $(c_1,k,m_2,s)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt2} Sample encryption $c_2\gets\E.\Enc(k,m)$.
      \item If $\Ext(c_1,c_2)=s$, then output $c_2$. Else, go back to step \ref{itm:encrypt2}.
    \end{enumerate}
  \item $\Sigma^{\E,\TwoExt}.\Seek$ takes as input $(k',c_1,c_2)$ and outputs $s':=\Ext(c_1,c_2)$.
\end{itemize}
\end{definition}

\begin{remark}
The schemes of Definitions \ref{def:ext_rejsampling} and \ref{def:2ext_rejsampling} are only \emph{expected} polynomial time.
They could straightforwardly be modified to run in polynomial time, by setting a polynomial upper bound on the number of attempted encryptions.
For an appropriate setting of this upper bound (e.g., $\ell^2$),
the distance between the output distribution of the original and modified (upper-bounded) algorithms would be negligible.
\end{remark}

\begin{proposition}
	Let $\E$, $\TwoExt$ and $\Sigma^{E,\TwoExt}$ be as in
	Definition~\ref{def:2ext_rejsampling}. Let us define
	$\scU\defeq\{U_{\ell(\kappa)}\}_{\kappa\in\NN}$. Assume that $\E$ is
	a semantically secure public-key encryption scheme and that $\TwoExt$ is
	a secure two-source extractor for identical sources, then
	$\Sigma^{\E,\TwoExt}$ is $\scU$-hiding for $\E$. Furthermore, if $\TwoExt$
	is strong, the $\Sigma^{\E,\TwoExt}$ is correct.
\end{proposition}

\begin{proof}
	We prove the proposition for $N=1$, the generalization to an arbitrary
	polynomial $N$ follows from a standard hybrid argument.

	Let us define the following random variables:
	\begin{align*}
		(PK, SK)\sim\PKE.\Gen(1^\kappa)\quad&
		(Z_0,Z_1)\stackrel{i.i.d}\sim \PKE.\Enc(1^\kappa) \\
		C_{0,1}\sim\PKE.\Enc(PK,m_1)
		\quad C_{1,1}&\sim\Sigma^{\E,\TwoExt}.\Hide_1(PK, m_1, U_\ell)\\
		C_{0,2}\sim\PKE.\Enc(PK, m_2)
		\quad C_{1,2}&\sim\Sigma^{\E,\TwoExt}.\Hide_2(C_{1,1}, PK, m_2, U_\ell)
	\end{align*}

	First, we note that by definition $\Sigma.\Hide_1$, $C_{0,1}\sim C_{1,1}$,
	and by definition of $\Sigma.\Hide_2$, if $C_{0,2}'$ is an independent copy
	of $C_{0,2}$, then:
	\begin{equation}
		\label{eq:rej}
		C_{0,2}\sim\Sigma^{\E,\TwoExt}.\Hide_2\big(C_{1,1}, PK, m_2,
		\TwoExt(C_{1,1}, C_{0,2}')\big)
	\end{equation}
	We also have:
	\begin{displaymath}
		\TwoExt(C_{1,1}, C_{0,2}')\compIndist\TwoExt(Z_0, Z_1)
		\statIndist U_{\ell}
	\end{displaymath}
	where the first approximation follows from semantic security and the second
	follows from Lemma~\ref{lemma:2ext}. This implies with \eqref{eq:rej} that
	$C_{0,2}\compIndist C_{1,2}$ and $(C_{0,1}, C_{0,2})\compIndist (C_{1,1},
	C_{1,2})$, which concludes the proof that $\Sigma$ is hiding.
\end{proof}











\section{Model and definitions}


For simplicity, we only consider conversations involving two parties, $A$ and $B$,
but our results extend to conversations between multiple parties.
We assume a synchronous communication model in which every party may send a message in every round.
A communication \emph{transcript} consists of a list of the messages
sent by each party for a number of consecutive rounds of communication.
We assume there is a PKI that provides a unique public identifier to each party.

\begin{definition}[Next-message algorithm]
A \emph{next-message algorithm} $\Next$ for message space $\Msg$
is a PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
and outputs a ``next message'' $m\in\Msg\cup\{\bot\}$, where the $\bot$ symbol denotes that no message is to be sent in the next round.
\end{definition}

%\begin{definition}[Next-ciphertext algorithm]
%For any encryption scheme $\E$, we denote by $\Next^{\E,k}$ the PPT algorithm that takes as input a (plaintext) communication transcript $\tau$,
%samples $m\gets\Next(\tau)$, and outputs an encryption $\E.\Enc(k,m)$.
%\end{definition}

\begin{definition}[Plaintext conversation distribution]
%Let $\PKE$ be a public-key encryption scheme and
Let $(A,B)$ be a pair of parties with public keys $pk_A,pk_B$ respectively,
and with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Then there is induced a unique \emph{$N$-round conversation distribution} $\Convo_{N,\Nextvec}$
defined by the following sampling procedure:

\begin{enumerate}
\item Initialize $\btau:=()$ to be an empty list.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  %\item\label{step:msg_i} Let $\tau_i:=(m_A,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \end{enumerate}
\item Output $\btau$.
\end{enumerate}
\end{definition}

\begin{definition}[Encrypted conversation distribution]
Let $(A,B)$ be a pair of parties %with public keys $pk_A,pk_B$ respectively,
with associated next-message algorithms ${\Nextvec}=(\Next_A,\Next_B)$.
Let $\E$ be an encryption scheme and let $k_A,k_B$ be encryption keys thereof.
There is induced an \emph{$N$-round encrypted conversation distribution} $\Convo_{N,\Nextvec}^{\E,k_A,k_B}$
defined by the following sampling procedure:
%same message-sampling procedure as above, except with step \ref{step:msg_i} replaced by the following:
%\begin{itemize}
%\item Sample $c_A\gets\PKE.\Enc(pk_B,m_A)$ and $c_B\gets\PKE.\Enc(pk_A,m_B)$ and let $\tau_i:=(c_A,c_B)$.
%\end{itemize}

\begin{enumerate}
\item Initialize $\btau:=(),\btau':=()$.
\item For each round $i=1,\dots,N$ of communication:
  \begin{enumerate}
  \item Sample $m_A\gets\Next_A(\btau)$ and $m_B\gets\Next_B(\btau)$.
  \item Sample $c_A\gets\SKE.\Enc(sk,m_A)$ and $c_B\gets\SKE.\Enc(sk,m_B)$.
  \item Append $(m_A,m_B)$ to the (plaintext) transcript $\btau$.
  \item Append $(c_A,c_B)$ to the (encrypted) transcript $\btau'$.
  \end{enumerate}
\item Output $\btau'$.
\end{enumerate}
\end{definition}

\subsection{Embedding into one ciphertext at a time}

\begin{definition}[Simple embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$.
A \emph{simple embedding scheme for strings of length $\ell$} is a pair of algorithms $\Sigma=(\Sigma.\Hide,\Sigma.\Seek)$ as follows.
\begin{itemize}
  \item $\Sigma.\Hide$ takes as input a key $k$, message $m\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs a ciphertext $c\in\Ciph_\kappa$.
  \item $\Sigma.\Seek$ takes as input a key $k'$ and a ciphertext $c\in\Ciph_\kappa$, and outputs a string $s'\in\zo^{\ell(\kappa)}$.
\end{itemize}
%We say that $\Sigma$ is \emph{secure w.r.t. $\SKE$ (respectively, $\PKE$)}
%if it is \emph{correct} and \emph{hiding} w.r.t. $\SKE$ (respectively, $\PKE$) as defined below.
\end{definition}

\begin{definition}[Correctness of simple embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$,
and let $\Sigma$ be a simple embedding scheme for strings of length $\ell=\ell(\kappa)$.
\begin{itemize}
  \item $\Sigma$ is \emph{correct w.r.t. $\SKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell,m\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    sk\gets\SKE.\Gen(1^\kappa) \\
    c\gets\Sigma.\Hide(sk,m,s) \\
    s'\gets\Sigma.\Seek(sk,c)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
  \item $\Sigma$ is \emph{correct w.r.t. $\PKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell,m\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    (pk,sk)\gets\PKE.\Gen(1^\kappa) \\
    c\gets\Sigma.\Hide(pk,m,s) \\
    s'\gets\Sigma.\Seek(sk,c)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
\end{itemize}
\end{definition}

\begin{definition}[Hiding of simple embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
A simple embedding scheme $\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\SKE.\Enc(sk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(sk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\PKE.\Enc(pk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(pk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}

\subsection{Adaptive embedding into pairs of ciphertexts}

\begin{definition}[Two-part embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$.
A \emph{two-part embedding scheme for strings of length $\ell$} is a triple of algorithms $\Sigma=(\Sigma.\Hide_1,\Sigma.\Hide_2,\Sigma.\Seek)$ as follows.
\begin{itemize}
  \item $\Sigma.\Hide_1$ takes as input a key $k$, message $m_1\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs $(c_1,\state)$ where $c_1\in\Ciph_\kappa$ is a ciphertext and $\state\in\zo^*$ is a \emph{state}.
  \item $\Sigma.\Hide_2$ takes as input a state $\state$, a key $k$, message $m_2\in\Msg_\kappa$, a string $s\in\zo^{\ell(\kappa)}$, and outputs a ciphertext $c_2\in\Ciph_\kappa$.
  \item $\Sigma.\Seek$ takes as input a key $k$ and ciphertexts $c_1,c_2\in\Ciph_\kappa)$, and outputs a string $s'\in\zo^{\ell(\kappa)}$.
\end{itemize}
\end{definition}

\begin{definition}[Correctness of two-part embedding scheme]
Let $\SKE,\PKE$ be secret- and public-key encryption schemes, respectively, each with message space $\Msg$ and ciphertext space $\Ciph$,
and let $\Sigma$ be a two-part embedding scheme for strings of length $\ell=\ell(\kappa)$.
\begin{itemize}
  \item $\Sigma$ is \emph{correct w.r.t. $\SKE$} if there is a negligible function $\eps$ such that $\forall s\in\zo^\ell$ and $m_1,m_2\in\Msg_k$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    sk\gets\SKE.\Gen(1^\kappa) \\
    (c_1,\state)\gets\Sigma.\Hide_1(sk,m_1,s) \\
    c_2\gets\Sigma.\Hide_2(\state,sk,m_2,s) \\
    s'\gets\Sigma.\Seek(sk,c_1,c_2)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
  \item $\Sigma$ is \emph{correct w.r.t. $\PKE$} if there is a negligible function $\eps$ such that for all $s\in\zo^\ell$,
    $$
    \Pr\left[
    \begin{array}{lll}
    \begin{array}{l}
    (pk,sk)\gets\PKE.\Gen(1^\kappa) \\
    (c_1,\state)\gets\Sigma.\Hide_1(pk,m_1,s) \\
    c_2\gets\Sigma.\Hide_2(\state,pk,m_2,s) \\
    s'\gets\Sigma.\Seek(sk,c_1,c_2)
    \end{array}
    &:&
    s'=s
    \end{array}
    \right] > 1- \eps(\kappa)\ .
    $$
\end{itemize}
\end{definition}

\begin{definition}[Hiding of two-part embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
A two-part embedding scheme $\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $((m_{1,1},m_{1,2}),\dots,(m_{N,1},m_{N,2}))\in((\Msg_\kappa)^2)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_{0,1}\gets\SKE.\Enc(sk,m_{i,1}) \\
\forall i\in[N], ~ c^{(i)}_{0,2}\gets\SKE.\Enc(sk,m_{i,2}) \\
\forall i\in[N], ~ (c^{(i)}_{1,1},\state_i)\gets\Sigma.\Hide_1(sk,m_{i,1},s_i) \\
\forall i\in[N], ~ c^{(i)}_{1,2}\gets\Sigma.\Hide_2(\state_i,sk,m_{i,2},s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $((m_{1,1},m_{1,2}),\dots,(m_{N,1},m_{N,2}))\in((\Msg_\kappa)^2)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_{0,1}\gets\PKE.\Enc(pk,m_{i,1}) \\
\forall i\in[N], ~ c^{(i)}_{0,2}\gets\PKE.\Enc(pk,m_{i,2}) \\
\forall i\in[N], ~ (c^{(i)}_{1,1},\state_i)\gets\Sigma.\Hide_1(pk,m_{i,1},s_i) \\
\forall i\in[N], ~ c^{(i)}_{1,2}\gets\Sigma.\Hide_2(\state_i,pk,m_{i,2},s_i) \\
b'\gets\sD(sk,(c^{(1)}_{b,1},c^{(1)}_{b,2}),\dots,(c^{(N)}_{b,1},c^{(N)}_{b,2})) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}

\begin{remark}
One could consider extending this definition to embed in more than polynomially many (rather than just two) ciphertexts at a time.
\sunoo{mention why adaptivity is important}
\end{remark}

\iffalse
\begin{definition}[Hiding of string-embedding scheme]
Let $N=N(\kappa)$ be a polynomial, let $\ell=\ell(\kappa)$,
and let $\scS=\{\scS_\kappa\}_{\kappa\in\NN}$ be a family of distributions, where each $\scS_\kappa$ is a distribution over $(\zo^{\ell})^N$.
$\Sigma$ is \emph{$\scS$-hiding for $\SKE$} if for any messages $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$ and
any PPT distinguisher $\sD$, there is a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
sk\gets\SKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\SKE.\Enc(sk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(sk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
Similarly, $\Sigma$ is \emph{$\scS$-hiding for $\PKE$} for any $(m_1,\dots,m_N)\in(\Msg_\kappa)^N$, and
any PPT distinguisher $\sD$, $\exists$ negligible $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
b\gets\zo \\
(s_1,\dots,s_N)\gets \scS_k \\
\forall i\in[N], ~ c^{(i)}_0\gets\PKE.\Enc(pk,m_i) \\
\forall i\in[N], ~ c^{(i)}_1\gets\Sigma.\Hide(pk,m_i,s_i) \\
b'\gets\sD(sk,c^{(1)}_b,\dots,c^{(N)}_b) \\
\end{array}
&:&
b'=b
\end{array}
\right] < \frac{1}{2} + \eps(\kappa)\ .
$$
\end{definition}
\fi

\subsection{Embedding schemes based on extractors}

\begin{definition}\label{def:ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^c$, and let
	$\Ext:\zo^c\to\zo^\ell$ be a deterministic extractor.
We define a simple embedding scheme $\Sigma^{\E,\Ext}$ for strings of length $\ell$, as follows.
\begin{itemize}
  \item $\Sigma^{\E,\Ext}.\Hide$ takes as input $(k,m,s)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt1} Sample encryption $c\gets\E.\Enc(k,m)$.
      \item If $\Ext(c)=s$, then output $c$. Else, go back to step \ref{itm:encrypt1}.
    \end{enumerate}
  \item $\Sigma^{\E,\Ext}.\Seek$ takes as input $(k',c)$ and outputs $s':=\Ext(c)$.
\end{itemize}
\end{definition}

\begin{definition}\label{def:2ext_rejsampling}
	Let $\E$ be an encryption scheme with ciphertext space $\zo^c$, and let
	$\TwoExt:\zo^c\times\zo^c\to\zo^\ell$ be a two-source extractor.
	We define
	a string-embedding scheme $\Sigma^{\E,\TwoExt}$ for strings of length
	$\ell$, as follows.
\begin{itemize}
  \item $\Sigma^{\E,\TwoExt}.\Hide_1$ takes as input $(k,m_1,s)$, samples $c_1\gets\E.\Enc(k,m)$, and outputs $(c_1,c_1)$.
  \item $\Sigma^{\E,\TwoExt}.\Hide_2$ takes as input $(c_1,k,m_2,s)$, and runs as follows:
    \begin{enumerate}
      \item\label{itm:encrypt2} Sample encryption $c_2\gets\E.\Enc(k,m)$.
      \item If $\Ext(c_1,c_2)=s$, then output $c_2$. Else, go back to step \ref{itm:encrypt2}.
    \end{enumerate}
  \item $\Sigma^{\E,\TwoExt}.\Seek$ takes as input $(k',c_1,c_2)$ and outputs $s':=\Ext(c_1,c_2)$.
\end{itemize}
\end{definition}

\begin{remark}
The schemes of Definitions \ref{def:ext_rejsampling} and \ref{def:2ext_rejsampling} are only \emph{expected} polynomial time.
They could straightforwardly be modified to run in polynomial time, by setting a polynomial upper bound on the number of attempted encryptions.
For an appropriate setting of this upper bound (e.g., $\ell^2$),
the distance between the output distribution of the original and modified (upper-bounded) algorithms would be negligible.
\end{remark}

\begin{proposition}
	Let $\E$, $\TwoExt$ and $\Sigma^{E,\TwoExt}$ be as in
	Definition~\ref{def:2ext_rejsampling}. Let us define
	$\scU\defeq\{U_{\ell(\kappa)}\}_{\kappa\in\NN}$. Assume that $\E$ is
	a semantically secure public-key encryption scheme and that $\TwoExt$ is
	a secure two-source extractor for identical sources, then
	$\Sigma^{\E,\TwoExt}$ is $\scU$-hiding for $\E$. Furthermore, if $\TwoExt$
	is strong, the $\Sigma^{\E,\TwoExt}$ is correct.
\end{proposition}

\begin{proof}
	We prove the proposition for $N=1$, the generalization to an arbitrary
	polynomial $N$ follows from a standard hybrid argument.

	Let us define the following random variables:
	\begin{align*}
		(PK, SK)\sim\PKE.\Gen(1^\kappa)\quad&
		(Z_0,Z_1)\stackrel{i.i.d}\sim \PKE.\Enc(1^\kappa) \\
		C_{0,1}\sim\PKE.\Enc(PK,m_1)
		\quad C_{1,1}&\sim\Sigma^{\E,\TwoExt}.\Hide_1(PK, m_1, U_\ell)\\
		C_{0,2}\sim\PKE.\Enc(PK, m_2)
		\quad C_{1,2}&\sim\Sigma^{\E,\TwoExt}.\Hide_2(C_{1,1}, PK, m_2, U_\ell)
	\end{align*}

	First, we note that by definition $\Sigma.\Hide_1$, $C_{0,1}\sim C_{1,1}$,
	and by definition of $\Sigma.\Hide_2$, if $C_{0,2}'$ is an independent copy
	of $C_{0,2}$, then:
	\begin{equation}
		\label{eq:rej}
		C_{0,2}\sim\Sigma^{\E,\TwoExt}.\Hide_2\big(C_{1,1}, PK, m_2,
		\TwoExt(C_{1,1}, C_{0,2}')\big)
	\end{equation}
	We also have:
	\begin{displaymath}
		\TwoExt(C_{1,1}, C_{0,2}')\compIndist\TwoExt(Z_0, Z_1)
		\statIndist U_{\ell}
	\end{displaymath}
	where the first approximation follows from semantic security and the second
	follows from Lemma~\ref{lemma:2ext}. This implies with \eqref{eq:rej} that
	$C_{0,2}\compIndist C_{1,2}$ and $(C_{0,1}, C_{0,2})\compIndist (C_{1,1},
	C_{1,2})$, which concludes the proof that $\Sigma$ is hiding.
\end{proof}


==> sections/silas_prelims.tex <==

\section{Preliminaries}

$\kappa$ is the security parameter throughout.
PPT means ``probabilistic polynomial time.''

\paragraph{Notation.}
$[n]$ denotes the set $\{1,\ldots, n\}$. $U_n$ is a uniform variable over
$\zo^n$ independent of every other variable in this paper. We write $X\sim Y$
to express that $X$ and $Y$ are identically distributed. Given two variables
$X$ and $Y$ over $\zo^k$, we denote by $\sdist{X - Y}$ the statistical distance
between $X$ and $Y$ defined by:
	\begin{displaymath}
		\begin{split}
			\sdist{X-Y}
			&=\frac{1}{2}\sum_{x\in\zo^k}\big|\Pr[X=x] - \Pr[Y=x]\big|\\
			&=\max_{S\subseteq\zo^k}\big|\Pr[X\in S]-\Pr[Y\in S]\big|.
		\end{split}
	\end{displaymath}
For a random variable $X$ of finite support, we define the min-entropy $\Me(X)$
of $X$ by $\Me(X)=-\log\max_{x} \Pr[X=x]$. The collision probability is
$CP(X)\defeq\sum_x\Pr[X=x]^2$. We will make repeated use of the standard
inequalities:
\begin{displaymath}
	\frac{1}{2^{2\Me(X)}}\leq CP(X)\leq \frac{1}{2^{\Me(X)}}
\end{displaymath}
\begin{displaymath}
	CP(X)-\frac{1}{2^n}
	\leq\sdist{X-U_n}^2
	\leq 2^n \left(CP(X)-\frac{1}{2^n}\right)
\end{displaymath}

\paragraph{Public/Private-Key Encryption.}
We assume familiarity with the standard notions of semantically secure public-key and private-key encryption.  We use the notation $\E=(\E.\Gen,\E.\Enc,\E.\Dec)$ for the backdoored public-key encryption scheme.  Our main construction will use a secret-key encryption scheme $\SKE=(\Gen,\Enc,\Dec)$ with pseudorandom ciphertexts as a building block.  Such secret-key encryption schemes can be built from any one-way function.

\paragraph{$\E-$Protocols.}
We say that a two party protocol between parties $P_1$ and $P_2$ with public keys $\pk_1$ and $\pk_2$, is an $\E-$\emph{protocol} if every message from $P_1$ to $P_2$ (likewise, from $P_2$ to $P_1$) is an $\E-$ciphertext, encrypted to $\pk_2$ (likewise $\pk_1$).  We will denote the transcript of such a protocol $(c_1,c'_1,\dots,c_r)$; we assume $P_1$ speaks first and last so the $c_i$ are $\E-$encryptions to $\pk_2$, $c'_i$ are $\E-$encryptions to $\pk_1$.  In order to optimize rounds, parties can send more than one ciphertext at once, in which case the transcript is $\bigl(\{c_{1,\alpha}\}_\alpha,\{c_{1,\alpha}'\}_\alpha,\dots\bigr)$.  For notational simplicity we work with transcripts where each round consists of a single ciphertext; our definitions and assertions extend naturally to the more general case.

\paragraph{$\E-$Protocol Conversations.}
Let $m_i=\E.\Dec(\sk_2,c_i)$ and $m_i'=\E.\Dec(\sk_1,c_i')$.  We call $(m_1,m_1',\dots,m_r)$ the \emph{conversation} of the $\E-$protocol transcript $(c_1,c_1',\dots,c_r)$.  We stress that while $P_1$ and $P_2$ might use an $\E-$protocol to exchange information which has nothing to do with the transcript's conversation, they still must take care to produce a realistic-looking conversation.  This is because the conversation can be inferred from the transcript by any party who knows the secret keys, and we assume $\E$ is backdoored.  Thus, if the conversation appears unrealistic, $P_1$ and $P_2$ will be identified as communicating illegally.  Because of this, generating each message of an $\E-$protocol involves choosing a realistic-looking next conversation message $m_i$ and then generating an encryption $c_i$ of $m_i$.  We avoid formalizing what it means for a conversation to appear realistic; we consider this to be outside the scope of this paper.  However, we make one assumption about realistic-looking conversations: that they can always be extended in a realistic-looking way.  Specifically, given a realistic-looking conversation ${\sf conv} = (m_1,m_1',\dots,m_{i-1},m_{i-1}')$, there is a distribution $\mathcal{M}({\sf conv})$ which outputs a realistic-looking next message $m_i$.  We will construct several $\E-$protocols.  Our first makes no assumptions on $\mathcal{M}({\sf conv})$, we then give improvements which assume that $\mathcal{M}({\sf conv})$ has sufficient min-entropy.  This assumption, while not without loss of generality, in certain contexts might be rather benign (for example, if the messages exchanged between $P_1$ and $P_2$ are images).  We denote by $\mathcal{M}^r(\cdot)$ the distribution which outputs a length $r$ realistic-looking conversation $(m_1,m_1',\dots,m_r)$ by drawing each $m_i/m_i'\leftarrow\mathcal{M}(m_1,\dots,m_{i-1}'/m_i)$.


\iffalse
We define the syntax only (and refer to a textbook for standard correctness/security defs).

%\begin{definition}[Secret-key encryption scheme]
%A \emph{secret-key encryption scheme} over a message space $\Msg$
%and ciphertext space $\Ciph$ is a tuple of
%PPT algorithms $\SKE=(\SKE.\Gen,\SKE.\Enc,\SKE.\Dec)$ as follows.
%\begin{itemize}
%\item $\SKE.\Gen$ takes input $1^\kappa$ and outputs a secret key $sk$.
%\item $\SKE.\Enc$ takes as input a secret key $sk$ and a message $m\in\Msg$,
%and outputs a ciphertext $c\in\Ciph$.
%\item $\SKE.\Dec$ is a deterministic algorithm that takes as input
%a secret key $sk$ and a ciphertext $c$, and outputs a decryption $m'\in\Msg\cup\{\bot\}$.
%\end{itemize}
%\end{definition}

\begin{definition}[Secret-key encryption scheme]
A \emph{secret-key encryption scheme} over a message space $\Msg=\{\Msg_\kappa\}_{\kappa\in\NN}$
and ciphertext space $\Ciph=\{\Ciph_\kappa\}_{\kappa\in\NN}$ is a tuple of
PPT algorithms $\SKE=(\SKE.\Gen,\SKE.\Enc,\SKE.\Dec)$ as follows.
\begin{itemize}
\item $\SKE.\Gen$ takes input $1^\kappa$ and outputs a secret key $sk$.
\item $\SKE.\Enc$ takes as input $(1^\kappa,sk,m)$ where $sk$ is a secret key and $m\in\Msg_\kappa$ is a message,
and outputs a ciphertext $c\in\Ciph_\kappa$.
\item $\SKE.\Dec$ is a deterministic algorithm that takes as input $(1^\kappa,sk,c)$ where
$sk$ is a secret key and $c\in\Ciph_\kappa$ is a ciphertext, and outputs a decryption $m'\in\Msg_\kappa\cup\{\bot\}$.
\end{itemize}
\end{definition}

%\begin{definition}[Public-key encryption scheme]
%A \emph{public-key encryption scheme} over a message space $\Msg$ and ciphertext space $\Ciph$ is a tuple of PPT algorithms
%$\PKE=(\PKE.\Gen,\PKE.\Enc,\PKE.\Dec)$ as follows.
%\begin{itemize}
%  \item $\PKE.\Gen$ takes input $1^\kappa$ and outputs a key pair $(pk,sk)$.
%  \item $\PKE.\Enc$ takes as input a public key $pk$ and a message $m\in\Msg$
%    and outputs a ciphertext $c\in\Ciph$.
%  \item $\PKE.\Dec$ is a deterministic algorithm that takes
%    as input a ciphertext $c$ and a secret key $sk$, and outputs a decryption $m'\in\Msg\cup\{\bot\}$.
%\end{itemize}
%\end{definition}

\begin{definition}[Public-key encryption (PKE) scheme]
A \emph{public-key encryption scheme} over a message space $\Msg=\{\Msg_\kappa\}_{\kappa\in\NN}$
and ciphertext space $\Ciph=\{\Ciph_\kappa\}_{\kappa\in\NN}$ is a tuple of PPT algorithms
$\PKE=(\PKE.\Gen,\PKE.\Enc,\PKE.\Dec)$ as follows.
\begin{itemize}
  \item $\PKE.\Gen$ takes input $1^\kappa$ and outputs a key pair $(pk,sk)$.
  \item $\PKE.\Enc$ takes as input $(1^\kappa,pk,m)$ where $pk$ is a public key and $m\in\Msg_\kappa$ is a message,
and outputs a ciphertext $c\in\Ciph_\kappa$.
  \item $\PKE.\Dec$ is a deterministic algorithm that takes as input $(1^\kappa,sk,c)$ where
$sk$ is a secret key and $c\in\Ciph_\kappa$ is a ciphertext, and outputs a decryption $m'\in\Msg_\kappa\cup\{\bot\}$.
\end{itemize}
\end{definition}

\begin{definition}[CPA security of PKE]
Let $\PKE$ be a PKE.
For any message $m\in\cM$, for all PPT adversaries $\cA=(\cA_1,\cA_2)$, there exists a negligible function $\eps$ such that
$$
\Pr\left[
\begin{array}{lll}
\begin{array}{l}
(pk,sk)\gets\PKE.\Gen(1^\kappa) \\
(m_0,m_1,\state)\gets\cA_1(1^\kappa,pk) \\
b\gets\zo \\
c_0\gets\PKE.\Enc(pk,m_0) \\
c_1\gets\PKE.\Enc(pk,m_1) \\
b'\gets\cA_2(\state,c_b)
\end{array}
&:&
b'=b
\end{array}
\right] > 1/2 + \eps(\kappa)\ .
$$
\end{definition}

For both types of encryption schemes, the input $1^\kappa$ is often omitted and left implicit.
\fi

==> sections/subl-old.tex <==
\section{Subliminal Communication}
\label{sec:subl}

\subsection{Definition and Main Theorem}

\paragraph{Conversation model.} The protocols we will construct take place over
a communication between two parties $P_1$ and $P_2$ alternatingly exchanging
ciphertexts of a public-key encryption scheme. \emph{W.l.o.g.}, we
assume that $P_1$ initiates the communication and we denote by $m_i$ (resp.
$m_i'$) the plaintext message sent by $P_1$ to $P_2$ (resp. $P_2$ to $P_1$)
during round $i$.

Since we assume that the adversary can decrypt all ciphertexts, it is necessary
that the conversation between $P_1$ and $P_2$ appears realistic. Formally
defining ``realistic'' is beyond the scope of this paper; instead, we simply
assume that there exists a next-message distribution $\mathcal{M}$ which
outputs a realistic looking message given the transcript of the conversation so
far. Writing $\btau_i=(m_1,m_1',\dots,m_{i-1},m'_{i-1})$ and
$\btau_i'=(m_1,m_1',\dots,m_{i-1},m_{i-1}',m_i)$ the transcripts available to
$P_1$ and $P_2$ respectively during round $i$, we have
$m_i\gets\mathcal{M}(\btau_i)$ and $m_i'\gets\mathcal{M}(\btau_i')$. 

Our main construction of a subliminal scheme makes no assumptions on the
distribution $\mathcal{M}$ and in particular implies that it is possible to
subliminally embed a message in an \emph{arbitrary} discussion between $P_1$
and $P_2$ (\emph{e.g.} a discussion where a fixed message is repeatedly
exchanged). We later give an improved construction which assumes that
$\mathcal{M}$ has sufficient min-entropy.  This assumption, while not without
loss of generality, might be rather benign in certain contexts (for example, if
the messages exchanged are images).

\begin{definition}[Subliminal communication scheme]
\label{def:subliminal}
A subliminal communication scheme is a two-party protocol:
\begin{displaymath}
\Pi^\E=\bigl(\Pi_{1,1}^\E,\Pi^\E_{1,2},\Pi^\E_{2,1},\Pi^\E_{2,2},
	\dots,\Pi^\E_{r-1,1},\Pi^\E_{r-1,2},\Pi^\E_{r,1};\Pi^\E_{2,{\sf out}}\bigr)
\end{displaymath}
	where $r(\kappa)\in\poly(\kappa)$ and where each $\Pi^\E_{i,j}$ is a PPT
	algorithm with oracle access to a public-key encryption scheme $\E$. When
	there is a no ambiguity we will drop the superscript $\E$ and make the
	oracle access implicit. The protocol must satisfy the following syntax,
	correctness and security guarantees.

\begin{itemize}
\item \textbf{Syntax.} For each $\msg\in\{0,1\}^\kappa$, initialize
	$\state_0=\state'_0=\emptyset$, and for $i=1,\dots, r$:
	\begin{enumerate}
		\item $P_1$ draws $m_i\leftarrow\mathcal{M}(\btau_i)$ and
			$(c_i,\state_i)\leftarrow\Pi_{i,1}^\E(\msg,m_i,\pk_2,\state_{i-1})$ and sends
			$c_i$. 
		\item $P_2$ draws $m_i'\leftarrow\mathcal{M}(\btau_i')$ and
			$(c_i',\state_i')\leftarrow\Pi_{i,2}^\E(m_i',\pk_1,\state'_{i-1})$
			and sends $c_i'$. 
	\end{enumerate}
		After $r$ rounds, $P_2$ computes ${\sf msg}'=\Pi_{2,{\sf
		out}}^\E(\sk_2,\state_{r-1}')$ and halts.
		

\item\textbf{Correctness.} For any semantically secure encryption scheme $\E$,
	for any $\msg\in\{0,1\}^\kappa$, if $P_1$ and $P_2$
	play $\Pi^\E$ honestly, then $\msg'=\msg$ with probability
		$1-\negl(\kappa)$.
		The probability is taken over the random draws
		$(\pk_1,\sk_1)\gets\E.\Gen$, $(\pk_2,\sk_2)\gets\E.\Gen$ and the
		randomness of the protocol algorithms as well as the message
		distribution.

\item\textbf{Subliminal Indistinguishability.}
	For any semantically secure public-key encryption scheme $\E$, for any
		${\sf msg}\in\{0,1\}^\kappa$ and for $(\pk_1,\sk_1)\gets\E.\Gen$,
		$(\pk_2,\sk_2)\gets\E.\Gen$, the following distributions are
		computationally indistinguishable:

\begin{center}
\begin{tabular}{|p{0.42 \textwidth}|p{0.42\textwidth}|}
\hline
\underline{${\sf Real}(\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}}
	& \underline{${\sf Subliminal}({\sf msg},\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} \\
for $i=1,\dots,r$:

	\quad $m_i,m_i'\gets\cM(\btau_i),\cM(\btau_i')$

	\quad $c_i\leftarrow\E.\Enc(\pk_2,m_i)$

	\quad $c_i'\leftarrow\E.\Enc(\pk_1,m_i')$ 

output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$ &
for $i=1,\dots,r$:

	\quad $m_i,m_i'\gets\cM(\btau_i),\cM(\btau_i')$

	\quad $(c_i,\state_i)\leftarrow\Pi_{i,1}^\E(\msg,m_i,\pk_2,\state_{i-1})$

	\quad $(c_i',\state_i')\leftarrow\Pi_{i,2}^\E(m_i',\pk_1,\state'_{i-1})$

output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$ \\
\hline
\end{tabular}
\end{center}
\end{itemize}
We call $\frac{\kappa}{2r-1}$ the \emph{subliminal rate} of the protocol $\Pi$: this
is the number of ciphertexts which must be sent back and forth between $P_1$
and $P_2$ in order to subliminally communicate a $\kappa$-bit message. 
\end{definition}

\begin{remark}
	All the protocols we will consider implicitely accumulate in their internal
	state $\state$, $\state'$ the messages exchanged between $P_1$ and $P_2$
	(both the plaintexts and the ciphertexts). As a consequence, each algorithm
	$\Pi_{i,j}$ has the current transcript of the conversation as part of its
	input.
\end{remark}
	
We are now ready to state the main theorem of this work.

%This is because we have simplified notation by assuming that only one ciphertext is sent in each round.  If instead $t$ ciphertexts are sent during each round, then the subliminal rate is $\kappa/(2rt-t)$.

\begin{theorem}
\label{thm:subl}
	Assume there exists a key-agreement protocol with pseudorandom messages,
	then there exists a subliminal communication scheme.
\end{theorem}

Most known key agreement protocols have pseudorandom (actually most have random) ciphertexts.  This is the case for example for the classical protocol of Diffie and Hellman.

\subsection{Impossibility Results}

Before giving our construction of a subliminal communication scheme, we prove
two impossibility theorems. The first one shows that subliminal communication
is not readily solved by steganographic constructions. Specifically, we show
that for a large class of steganographic schemes parametrized by a public
random string, the government can chose its encryption scheme as a function of
the public random string in a manner which breaks the steganographic scheme.

We will not formally define a steganographic scheme here, as our impossibility theorem applies broadly to any communication scheme with a certain property, and it suffices for our purposes to define this property: namely, that the decoding function of the scheme---the function computed by
the receiving party to retrieve the hidden information---retrieves a constant
number of bits of the hidden information when computed on a single stegotext (a
ciphertext in our case).  Note that this class of steganographic schemes
contains in particular the constructions from \cite{AH04}.

\begin{theorem}
	\label{thm:impossibility-1}
	For any steganographic scheme of the type described above, there exists
	a semantically secure encryption scheme $\E$ dependent on the public randomness
	of the steganographic scheme, such that the number of bits of hidden
	information which can be steganographically embedded in ciphertexts of $\E$
	is arbitrarily small.
\end{theorem}
	
\begin{proof}
	Let us consider a steganographic scheme such as in the statement of the
	theorem and let us denote by $f:\zo^n\times\zo^m\to\zo$ the decoding
	function of the scheme. Without loss of generality, we assume that $f(s, r)$
	retrieves a single bit of hidden information when computed on stegotext $s$
	and public randomness $r$. Since we allow the encryption scheme to depend
	on the public randomness of the steganographic scheme, define the partial
	function $f_r(s) = f(s, r)$. $f_r$ is now a deterministic function of the
	stegotext and we conclude the proof by constructing an encryption scheme
	which biases the output of $f_r$ arbitrarily close to a constant bit.

	Let $\E,$ be a semantically secure encryption scheme with ciphertext space
	$\Ciph=\zo^n$ and message space $\Msg$. Without loss of generality we
	assume that for at least half the messages $m\in\Msg$, we have
	$\Pr[f_r(C_m)=1]\geq\frac{1}{2}$ (otherwise we can just replace 1 by
	0 in the construction below). We now define the encryption scheme $\E'$
	  which is identical to $\E$ except for $\E'.\Enc$ which on input $(pk, m)$
	  runs as follows for some constant $t$:

		\begin{enumerate}
		 \item Repeat at most $t$ times:
			\begin{enumerate}
				\item Sample encryption $c\gets\E.\Enc(pk, m)$.
				\item If $f_r(c)=1$ exit the loop otherwise continue.
			\end{enumerate}
		\item output $c$
		\end{enumerate}

	It is clear that $\E'$ is also semantically secure: oracle access to
	$\E'.\Enc$ can be simulated with oracle access to $\E.\Enc$, so
	a distinguisher which breaks the semantic security of $\E'$ can also be
	used to break the semantic security of $\E$. Finally, for a message $m$
	such that $\Pr[f_r(C_m)=1]\geq\frac{1}{2}$, by definition of
	$\E'.\Enc$:
	\begin{displaymath}
		\Pr[f_r(\E'.\Enc(PK, m))=1]\geq1-\frac{1}{2^t}
	\end{displaymath}
	which shows that the output of $f_r$ can be arbitrarily biased and
	concludes the proof.
\end{proof}

Our second impossibility theorem shows that subliminal communication is
impossible if we only assume that the cover distribution has a constant amount
of conditional min-entropy as is typically assumed in the provably secure
steganography literature. As already mentioned in the introduction, an
interesting feature of our work is to exhibit a situation where the cover
distribution is well-specified and whose structure can be exploited to
construct subliminal communication schemes despite the impossibility results
presented in this section.

\begin{theorem}
	\label{thm:impossibility-2}
No subliminal  communication scheme can satisfy all of the following properties
	simultaneously, for any $k$:
\begin{itemize}
\item requires no trusted setup;
\item allows the transmission of more than 1 hidden bit of information; and
\item works for all distributions of cover objects that have conditional min-entropy $k$.
\end{itemize}
\end{theorem}

\begin{proof}
	The proof is similar to the proof of the previous impossibility theorem,
	but instead of exploiting the impossibility of deterministic single source
	extraction, we exploit the impossibility of extracting more than one bit
	from Santha-Vazirani (SV) sources (cf. Proposition 6.6 in \cite{vad10}).
	Recall that a $\delta$-SV source $X\in\zo^n$ is defined by:
	\begin{displaymath}
		\delta\leq \Pr[X_i=1\,|\,X_1=x_1,\dots,X_{i-1}=x_{i-1}]\leq 1-\delta
	\end{displaymath}
	for all $i\in[n]$ and all $(x_1,\dots,x_{i-1})\in\zo^{i-1}$.

	Let us now consider a specific subliminal communication scheme satisfying
	the conditions of the theorem. Since the scheme requires no trusted setup,
	its decoding function $\Pi_{2,\sf out}$ is a fixed function. Let us now fix
	$\delta>0$, we can find $n\in\NN$ such that $\delta$-SV sources of length
	$n$ have min-entropy $k$. Applying Proposition 6.6 then implies that for any
	predicate $B$, there exists a $\delta$-SV source of min-entropy $k$ such
	that  $\Pr[B\big(\Pi_{2,\sf out}(X)\big) = 1] \geq 1-\delta$ or 
	$\Pr[B\big(\Pi_{2,\sf out}(X)\big) = 0] \geq 1-\delta$. By subliminal
	indistinguishability, this implies that the entropy of the decoding output
	is at most $1-\delta+\eps$ for some negligible $\eps$. For an appropriate
	choice of $\delta$ this limits the transmission of hidden information to
	less than 1 bit.
\end{proof}


==> sections/subldef.tex <==

\section{Subliminal Communication}
\begin{definition}
\label{def:subliminal}
We say that a public-key encryption scheme $\E$ \emph{supports subliminal communication} if there exists a polynomial $r=r(\kappa)$ and a two-party $\E-$protocol $$\Pi=\bigl(\Pi_{1,1},\Pi_{1,2},\Pi_{2,1},\Pi_{2,2},\dots,\Pi_{r-1,1},\Pi_{r-1,2},\Pi_{r,1};\Pi_{2,{\sf out}}\bigr)$$ for $\kappa-$bit message transmission with the following syntax, correctness and security guarantees.

\begin{itemize}
\item \textbf{Syntax.} For each $i=1,\dots,r$, and ${\sf msg}\in\{0,1\}^\kappa$, $P_1$ draws $m_i\leftarrow\mathcal{M}(m_1,\dots,m_{i-1}')$ and $c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(\pk_1,\sk_1,\pk_2);(c_1,\dots,c_{i-1}')\bigr)$ and sends $c_i$.  Likewise for $i=1,\dots,r-1$, $P_2$ draws $m_i'\leftarrow\mathcal{M}(m_1,\dots,m_i)$ and $c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(\pk_2,\sk_2,\pk_1);(c_1,\dots,c_i)\bigr)$ and sends $c_i'$.  After $r$ rounds, $P_2$ computes ${\sf msg}'=\Pi_{2,{\sf out}}\bigl(\sk_2;(c_1,\dots,c_r)\bigr)$ and halts.

\item\textbf{Correctness.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, if $P_1$ and $P_2$ play $\Pi$ honestly, ${\sf msg}'={\sf msg}$ with probability $1-\negl(\kappa)$.

\item\textbf{Subliminal Indistinguishability.} For any ${\sf msg}\in\{0,1\}^\kappa$ and key pairs $(\pk_1,\sk_1)$, $(\pk_2,\sk_2)$ for $\E$, the following distributions are indistinguishable:

\begin{center}
\begin{tabular}{|p{0.4 \textwidth}|p{0.4\textwidth}|}
\hline
\underline{${\sf Real}(\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} & \underline{${\sf Subliminal}({\sf msg},\pk_1,\sk_1,\pk_2,\sk_2)${\bf :}} \\
{$(m_1,m_1',\dots,m_r)\leftarrow\mathcal{M}^r(\cdot)$ \newline
$c_i/c_i'\leftarrow\E.\Enc(\pk_2/\pk_1,m_i/m_i')$ \newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} &
{$m_i/m_i'\leftarrow\mathcal{M}(m_1,m_1',\dots,m_{i-1}'/m_i)$\newline
$c_i\leftarrow\Pi_{i,1}\bigl({\sf msg};m_i;(c_1,\dots,c_{i-1}')\bigr)$\newline
$c_i'\leftarrow\Pi_{i,2}\bigl(m_i';(c_1,\dots,c_i)\bigr)$\newline
output $\bigl(\pk_1,\sk_1,\pk_2,\sk_2;(c_1,c_1',\dots,c_r)\bigr)$} \\
\hline
\end{tabular}
\end{center}
\end{itemize}
\end{definition}

We call $\kappa/(2r-1)$ the \emph{subliminal rate} of the $\E-$protocol $\Pi$.  Note that $(2r-1)$ is the number of $\E-$ciphertexts which must be sent back and forth between $P_1$ and $P_2$ in order to subliminally communicate a $\kappa-$bit message.
